Interpreting Attention Models with Human Visual Attention in Machine Reading Comprehension

While neural networks with attention mechanisms have achieved superior performance on many natural language processing tasks, it remains unclear to which extent learned attention resembles human visual attention. In this paper, we propose a new method that leverages eye-tracking data to investigate the relationship between human visual attention and neural attention in machine reading comprehension. To this end, we introduce a novel 23 participant eye tracking dataset - MQA-RC, in which participants read movie plots and answered pre-defined questions. We compare state of the art networks based on long short-term memory (LSTM), convolutional neural models (CNN) and XLNet Transformer architectures. We find that higher similarity to human attention and performance significantly correlates to the LSTM and CNN models. However, we show this relationship does not hold true for the XLNet models -- despite the fact that the XLNet performs best on this challenging task. Our results suggest that different architectures seem to learn rather different neural attention strategies and similarity of neural to human attention does not guarantee best performance.

==> sections/method.tex <==
%In this section we introduce the measure we use to calculate similarity between human and neural attention and the necessary preprocessing steps.

In order to compare the human and neural attention distributions, we identified the Kullback-Leibler Divergence~\cite{kullback1951information} to be the most suitable comparison method.

This method is used to compare two probability distributions, akin to relative entropy. We need to ensure we compare the two distributions in a specific and consistent order; meaning we can compare either H to M or M to H, but we cannot interchange this direction. Additionally, the information we gain from this measure is an understanding of the differences in probability distribution between two variables (cf. Equation \ref{eq:KL_div}).

\begin{equation}
\label{eq:KL_div}
{\displaystyle D_{\text{KL}}(H\parallel M)=\sum _{x\in {\mathcal {X}}}P(x)\log \left({\frac {H(x)}{M(x)}}\right).}
\end{equation}

%TODO INSERT THE KL DIVERGENCE BETWEEN PARTICIPANTS AS WELL, FIX THE WRITING OF IT A  BIT SUCH THAT WE MOTIVATE IN THE ABOVE SECTION AND EXPAND HERE WITH THE BETWEEN PTS RESULTS

Concretely, we calculate the KL divergence for average-human to average-model along the word level attention distributions. 

%In order to use this information, the following section discusses how we normalize in order to accommodate for the KL method. 

%Before the similarity between human and neural attention can be calculated, we have to transform them, in order to make them comparable (cf. section 6.2, 6.3, 6.4)

%After obtaining the difference score for each human participant and model, the numbers are averaged into a single number for each document.



